Decoding Brain Representations by Multimodal Learning of Neural Activity and Visual Features

This work presents a novel method of exploring human brain-visual representations, with a view towards replicating these processes in machines. The core idea is to learn plausible computational and biological representations by correlating human neural activity and natural images. Thus, we first propose a model, EEG-ChannelNet, to learn a brain manifold for EEG classification. After verifying that visual information can be extracted from EEG data, we introduce a multimodal approach that uses deep image and EEG encoders, trained in a siamese configuration, for learning a joint manifold that maximizes a compatibility measure between visual features and brain representations. We then carry out image classification and saliency detection on the learned manifold. Performance analyses show that our approach satisfactorily decodes visual information from neural signals. This, in turn, can be used to effectively supervise the training of deep learning models, as demonstrated by the high performance of image classification and saliency detection on out-of-training classes. The obtained results show that the learned brain-visual features lead to improved performance and simultaneously bring deep models more in line with cognitive neuroscience work related to visual perception and attention.

==> generation.tex <==
One of the most appealing application of being able to decode the human mind is probably that of reconstructing what is being seen in one's mind's eye. Without moving too far into science fiction (e.g., telepathy), examples of the usefulness of such a technique can be found in medicine, for instance as a means of communication for impaired people.

While we are still far from there, we can already formulate the reconstruction problem using existing techniques, such as generative adversarial networks (GAN)~\cite{gan}. In particular, using the compact representation provided by the proposed EEG encoder, we can guide the conditional generation of images that correspond to the information contained in an embedded EEG. This approach has been adopted in~\cite{iccv_eeg_gan} to generate reconstructions of image looked at by users from the EEG signals recorded during the experiment. In that case, however, the conditioning signals were generated by an EEG encoder trained explicitly for the GAN conditioning purpose, while in our case our EEG encoder is trained jointly with the image encoder, which makes it useful more generic analysis as well. Our objective in this experiment was therefore to train a conditional GAN framework, using our EEG encoder to provide the condition vectors, and compare the results with \cite{iccv_eeg_gan}. In particular, we employed the same metrics used in that work:
\begin{itemize}
 \item Inception score~\cite{inception_score} (IS): arguably the most used score for quantitatively evaluating GAN results, it analyzes the softmax output of a pre-trained Inception model~\cite{inception} to provides an indication on how recognizable and how diverse generated images are.
 \item{Inception classification accuracy} (IC): introduced in~\cite{iccv_eeg_gan}, this score consists in the classification accuracy obtained by a pre-trained Inception model on the images generated from a given label/condition. It provides an additional measure of how the content of the generated images resembles the corresponding visual class.
\end{itemize}

The design of our GAN architecture is strongly affected by the limited availability of images with associated EEG signals. Indeed, the employed dataset (described in Sect.~\ref{sec:dataset}) contains EEG signals associated to ``just'' 2000 images (which is a relatively large number of EEG datasets, but quite small --- especially considering that it includes 40 different visual classes --- for image datasets). However, given that the selected images come from ImageNet classes, which contain 1200-1300 images per class, there is a large bulk of images without corresponding EEG signals that could still be used for training. In~\cite{iccv_eeg_gan}, the authors initially train a conditional GAN model on all images of the selected classes, by zeroing the conditioning vector, and then fine-tune the model on the images with associated EEG signals, by using the output of a recurrent network as feature vector for conditioning. However, this training approach .........\textcolor{red}{reason why we changed approach}. For this reason, it is desirable to be able to jointly train the generator and discriminator both when a condition is provided and when it is not. Ideally, this means that the generator should learn how to generate realistic images in general, and how to generate a images with specific features when the condition is provided; similarly, the discriminator should learn how to distinguish between real and fake images in general, and how to verify that an image is both realistic and matches a certain condition, when such condition is provided.

Our GAN architecture is based on a conditional~\cite{cond_gan} variant of DCGAN~\cite{dcgan}, shown in Fig.~\ref{fig:gan_arch}. Our main modifications to the models are aimed at making the generator and discriminator suitable to deal with optional conditions, while maximizing the reuse of feature layers between the two modalities. To this end, the generator has an initial \emph{conditional} layer, which feeds the noise vector alone to a dedicated layer when no condition is provided, and the concatenated noise and condition to another layer when the condition is given. Both layers should have the same size, so that they can be interchangeably connected to the next layer, which ``merges'' the two paths so that all the following layers, which generate increasingly larger feature maps, can be shared by the computation. Similarly, the discriminator processes the input image through a cascade of layers, and the optional presence of a conditioning vector is evaluated at the final branch between a real/fake discrimination layer that only takes into account the features extracted from the image alone, and a real/fake discrimination layer which also takes into account the correct match between the visual features and the given condition.

While training this model, at each iteration we sample a real batch containing ``conditioned'' images only (i.e., with associated EEG signals, from which we compute a conditioning vector using the encoder trained in Sect.~\ref{sec:classification}) and a batch of ``unconditioned'' ones (the large majority of images). The discriminator is then trained with those batches (labeled as ``real''), plus the batch of conditioned images with wrong conditions (labeled as ``fake''), and a batch of generated images (labeled as ``fake'' as well). The generator is trained by computing the gradient of the discriminator loss when the latter is provided with both unconditioned and randomly-conditioned generated inputs and with randomly-conditioned generated, both labeled as real for the sake of loss computation. More formally, the losses employed while training the discriminator and the generator extend the traditional formulation by adding terms related to the double nature of what ``real'' and ``fake'' mean in the optionally-conditional context:
\begin{IEEEeqnarray}{lCl}
 \mathcal{L}_D & = & -\mathbb{E}_{x \sim p_{R_u}}\left[ \log D_u\left(x\right) \right] \\
\nonumber      &   & -\mathbb{E}_{x,c \sim p_{R_c}}\left[ \log D_c\left(x|c\right) \right] \\
\nonumber      &   & -\mathbb{E}_{x,w \sim p_{R_{w}}}\left[ \log \left( 1 - D_c\left( x|w \right) \right) \right] \\
\nonumber      &   & -\mathbb{E}_{z \sim p_z}\left[ \log \left( 1 - D_u\left( G_u\left(z\right) \right) \right) \right] \\
\nonumber      &   & -\mathbb{E}_{z \sim p_z,c \sim p_C}\left[ \log \left( 1 - D_c\left( G_c\left(z|c\right)|c \right) \right) \right]
\end{IEEEeqnarray}
\begin{IEEEeqnarray}{lCl}
 \mathcal{L}_G & = & -\mathbb{E}_{z \sim p_z}\left[ \log D_u\left(G_u\left( z \right) \right) \right] \\
\nonumber      & = & -\mathbb{E}_{z \sim p_z,c\sim p_C}\left[ \log D_c\left(G_c\left( z|c \right)|c\right) \right]
\end{IEEEeqnarray}
In the formulas above, $R_u$ is the set of unconditioned real images; $R_c$ is the set of pairs of real images with associated conditions; $R_{w}$ is the set of real images with associated \emph{wrong} conditions; $p_z$ is the noise distribution; $p_C$ is the distribution of conditioning vectors. Also, $D_u$ and $D_c$ respectively define the unconditional and conditional paths within the discriminator; the same goes for $G_u$ and $G_c$.

We train our models for 100 epochs with the Adam~\cite{adam} gradient descent algorithm with default hyperparameters, using mini-batches of size 64. The size of the input and generated images is 64$\times$64 pixels. Examples of generated images are shown in Fig.~\ref{fig:gen_examples}. A quantitative comparison with~\cite{iccv_eeg_gan}  terms of IS and IC scores is instead shown in Table~\ref{tab:gen_results}. The results show that the proposed approach is able to generate good quality samples --- remember that conditioning is performed through the output of EEG encoder --- and that the quality of generated images is comparable to that of~\cite{iccv_eeg_gan}, although the encoder our approach uses was trained in a more general way by maximizing a compatibility function between EEG signals and images. In our case, therefore, the success of the generation confirms that the EEG embedding, while not explicitly learned with class supervision \textcolor{red}{this is not actually true, because the loss function is a classification loss...}, is indeed able to encode visual information that allow to drive the generation of the correct type of image content.
